Construction of h-refined continuous finite element spaces with arbitrary hanging node configurations and applications to multigrid algorithms

We present a novel approach for the construction of basis functions to be employed in selective or adaptive h-refined finite element applications with arbitrary-level hanging node configurations. Our analysis is not restricted to $1$-irregular meshes, as it is usually done in the literature, allowing our results to be applicable to a broader class of local refinement strategies. The proposed method does not require the solution of any linear system to obtain the constraints necessary to enforce continuity of the basis functions and it can be easily implemented. A mathematical analysis is carried out to prove that the proposed basis functions are continuous and linearly independent. Finite element spaces are then defined as the spanning sets of such functions, and the implementation of a multigrid algorithm built on these spaces is discussed. A spectral analysis of the multigrid algorithm highlights superior convergence properties of the proposed method over existing strategies based on a local smoothing procedure. Finally, linear and nonlinear numerical examples are tested to show the robustness and versatility of the multigrid algorithm.

==> hanging nodes/shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{Construction of h-refined continuous finite element spaces with arbitrary hanging node configurations 
and applications to multigrid algorithms} 
\newcommand{\TheAuthors}{Eugenio Aulisa, Giacomo Capodaglio, Guoyi Ke}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors October 2, 2017.
\funding{This work was supported by the National Science Foundation grant DMS-1412796.}}}

% Authors: full names plus addresses.
\author{
  Eugenio Aulisa\thanks{Broadway \& Boston, Department of Mathematics and Statistics, Texas Tech University, Lubbock TX 79409, USA
    (\email{eugenio.aulisa@ttu.edu}),
    (\email{giacomo.capodaglio@ttu.edu}),
    (\email{guoyi.ke@ttu.edu}).}
  \and
  Giacomo Capodaglio \footnotemark[2]
  \and
  Guoyi Ke \footnotemark[2]
}

\headers{h-refined finite element spaces with hanging nodes}{Eugenio Aulisa, Giacomo Capodaglio, Guoyi Ke}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

